MDNet: Multi-Decoder Network for Abdominal CT Organs Segmentation

Accurate segmentation of organs from abdominal CT scans is essential for clinical applications such as diagnosis, treatment planning, and patient monitoring. To handle challenges of heterogeneity in organ shapes, sizes, and complex anatomical relationships, we propose a \textbf{\textit{\ac{MDNet}}}, an encoder-decoder network that uses the pre-trained \textit{MiT-B2} as the encoder and multiple different decoder networks. Each decoder network is connected to a different part of the encoder via a multi-scale feature enhancement dilated block. With each decoder, we increase the depth of the network iteratively and refine segmentation masks, enriching feature maps by integrating previous decoders' feature maps. To refine the feature map further, we also utilize the predicted masks from the previous decoder to the current decoder to provide spatial attention across foreground and background regions. MDNet effectively refines the segmentation mask with a high dice similarity coefficient (DSC) of 0.9013 and 0.9169 on the Liver Tumor segmentation (LiTS) and MSD Spleen datasets. Additionally, it reduces Hausdorff distance (HD) to 3.79 for the LiTS dataset and 2.26 for the spleen segmentation dataset, underscoring the precision of MDNet in capturing the complex contours. Moreover, \textit{\ac{MDNet}} is more interpretable and robust compared to the other baseline models.

==> takeout.tex <==
U-Net~\cite{ronneberger2015u}& & &	&	&	&\\
AttentionUNet~\cite{oktay2018attention}& & &	&	&	&\\
DeepLabV3+~\cite{chen2018encoder}	& & &	&	&	&\\
TransUNet~\cite{chen2021transunet}& & &	&	&	&\\
HiFormer~\cite{heidari2023hiformer}& & &	&	&	&\\
G-Cascade~\cite{rahman2024g}& & &	&	&	&\\
\textbf{MDNet (Ours)}& & &	&	&	&\\

%-----------------

Dynamic contrast-enhanced CT is a common technique for liver cancer diagnosis, where four different phases of imaging, namely, non-contrast (NC), arterial (ART), portal venous (PV), and delayed (DL) provide complementary information about the liver. 



we focus on organ segmentaion because it is one of the most critical tasks in medical image analysis. We 




Meanwhile, vision transformers (ViT) [4] have been shown to replace CNN with a transformer encoder in computer vision tasks and can achieve obvious advantages on large-scale datasets. To the best of our knowledge, we find no study using ViT backbone network in liver lesion classification. The reason for this is twofold. First, pure ViT has several limitations itself [6], including ignoring local information within each patch, extracting only single-scale features, and lacking inductive bias. Second, no complete open liver lesion classification datasets exist. Most relevant studies are based on private datasets, which tend to be small in size and cause overfitting in learning models.





% \paragraph{\textbf{Ablation study:}}
% \begin{table}[t!]
% \footnotesize
% \centering
% \caption{Ablation study results}
%  \begin{tabular} {l|c|c|c|c|c|c}
% \toprule
% \textbf{Method}  &\textbf{mDSC}  & \textbf{mIoU}   &\textbf{Recall}& \textbf{Precision} &\textbf{F2} &\textbf{HD} \\ 
% \hline
% Baseline & & & &	& &\\
% Baseline + DC Block  & & & & & &\\
% Baseline + MSFED Block & & & & & &\\
% Baseline + MA Block & & & &	& &\\
% Baseline + DC + MSFED Block & & & &	& &\\
% \textbf{MDNet (Ours)} &0.9169 &0.9504 &0.9577 &0.9567 &0.9538 &13.74\\
% \bottomrule
% \end{tabular}
% \label{tab:resultsKvasir-seg}
% \end{table}


%\subsection{Computational complexity analysis}



% \subsubsection*{Acknowledgement}
% This project is partially supported by the NIH funding: R01-CA246704 and R01-CA240639.


 routine medical images,

 heir performance to make better choices in diagnosis and treatment, and free their time to focus on giving patients the best care.”
 



% \begin{table}[t!]
% \footnotesize
% \centering
% \caption{Quantitative results of the model on  Liver MRI scan.}
%  \begin{tabular} {l|c|c|c|c|c|c}
% \toprule
% \textbf{Method}  &\textbf{mDSC}  & \textbf{mIoU}   &\textbf{Recall}& \textbf{Precision} &\textbf{F2} &\textbf{HD} \\ 
% \hline

% U-Net~\cite{ronneberger2015u}& & &	&	&	&\\
% AttentionUNet~\cite{oktay2018attention}& & &	&	&	&\\
% DeepLabV3+~\cite{chen2018encoder}	& & &	&	&	&\\
% TransUNet~\cite{chen2021transunet}& & &	&	&	&\\
% HiFormer~\cite{heidari2023hiformer}& & &	&	&	&\\
% G-Cascade~\cite{rahman2024g}& & &	&	&	&\\
% \textbf{B2 (Our)} & & &	&	&	&\\
% \bottomrule
% \end{tabular}
% \label{tab:resultsKvasir-seg}
% \end{table}
% %-----------------

% \begin{table}[t!]
% \footnotesize
% \centering
% \caption{Quantitative results of the model on Spleen MRI scan.}
%  \begin{tabular} {l|c|c|c|c|c|c}
% \toprule
% \textbf{Method}  &\textbf{mDSC}  & \textbf{mIoU}   &\textbf{Recall}& \textbf{Precision} &\textbf{F2} &\textbf{HD} \\ 
% \hline
% U-Net~\cite{ronneberger2015u}& & &	&	&	&\\
% AttentionUNet~\cite{oktay2018attention}& & &	&	&	&\\
% DeepLabV3+~\cite{chen2018encoder}	& & &	&	&	&\\
% TransUNet~\cite{chen2021transunet}& & &	&	&	&\\
% HiFormer~\cite{heidari2023hiformer}& & &	&	&	&\\
% G-Cascade~\cite{rahman2024g}& & &	&	&	&\\
% \textbf{MDNet (Ours)} & &	&	&	&\\
% \bottomrule
% \end{tabular}
% \label{tab:resultsKvasir-seg}
% \end{table}
% %-----------------



% Ours (MiT - B2) &\textbf{0.9169} &\textbf{0.9504} &\textbf{0.9577} &0.9567 &\textbf{0.9538} &\textbf{13.74} &20.81\\



%Ours (MiT - B3)	&0.8857	&0.9267	&0.9299	&0.9429	&0.9259	&32.89	&25.49\\
%Ours (MiT - B4)	&0.8907	&0.9283	&0.9309	&0.9518	&0.9279	&32.02	&19.76\\
%Ours (MiT - B5)	&0.8992	&0.9362	&0.9350	&0.9550	&0.9338	&30.81	&17.76\\


 GIF file for the abdominal 

https://github.com/MrGiovanni/SyntheticTumors 


Method check: (MDNet reputation)

sell interpretability (conclusion, discussion, results)

Network complexity (fps, no.of flops, parameters, )

attention unet & DeepLabv3+

related work add



%Each decoder progressively increases the number of decoder blocks. This progressive design enhances the network's complexity to facilitate learning complex representations. Notably, the output segmentation mask produced from each decoder is utilized in the subsequent decoder to provide spatial attention to the learned . 




% The first decoder begins with a $2\times2$ transpose convolution layer, where the spatial dimensions of the feature map $F_2$ are increased by a factor of two. Next, it is concatenated with the feature map $F_1$ and then followed by two residual block to learn the semantic features to generate a segmentation mask. Next, it is followed by a bilinear upsampling by a factor of four and then a $1\times1$ convolution and sigmoid activation function to generate the segmentation mask $M_1$.

% The first decoder consists of a single decoder block, which begins with $F_2$ as the input feature maps and $F_1$ as the skip connection. The output from the first decoder is followed by a bilinear upsampling having a factor of four and then a $1\times1$ convolution and sigmoid activation function to generate the segmentation mask $M_1$.

% The second and third decoder follows a similar structure and also utilize the Mask Attention (MA) block to further improve the feature representation and boost the segmentation performance. Additionally, same-scale feature maps the previous decoders are also utilized during the concatenation with the skip connection from the MiT-encoder. This helps in the propagation of the feature learned by the previous decoders which boost the performance. The second decoder consists of two decoder blocks, each followed by a Mask Attention block. It begins with a $2\times2$ transpose convolution layer, followed by a concatenation with the skip connection and then two residual block. The semantic features learned by the residual block are further enhanced by the Mask Attention block, which utilize $M_1$ and apply a foreground and background spatial attention parallelly to ehance the feature representation. The output from the Mask Attention block is then pass to the second decoder block, where same-scale feature from the first decoder along with MiT-encoder is concatenated and utilized as the skip connection. Next, it is again followed by the Mask Attention block which utilize $M_1$. The output from the second decoder is followed by a bilinear upsampling having a factor of four and then a $1\times1$ convolution and sigmoid activation function to generate the segmentation mask $M_2$. Similarly, we have third decoder which have three decoder blocks, each followed by a Mask Attention block. The output from the third decoder is upsampled, followed by a $1\times1$ convolutional layer and sigmoid activation to generate final segmentation mask $M_3$.


%This paper presents a novel approach for liver and spleen CT and MRI segmentation from abdominal CT and MRI examinations. 

%We propose a hybrid model called MDNet (Multi-Decoder Network) with a transformer backbone and complementary convolutional modules. The MDN architecture leverages a shared encoder to extract high-level features from input images, followed by multiple decoders, each dedicated to segmenting a specific organ. This multi-decoder approach allows for specialized feature learning tailored to the unique characteristics of each organ. At the same time, the shared encoder promotes the efficient utilization of computational resources and the extraction of common features relevant across organs. We perform extensive experiments on CT and MRI modalities for the liver and spleen. We achieved a dice coefficient of 0.9383 and mIoU of 0.9013, respectively. 


%Manual delineation of liver and spleen segments on CT scans is done by radiologists to understand the spread of the cancer for the appropriate treatment. However, 
